The Optimal Size and Progressivity of Old-Age Social Security

Almost every public pension system shares two attributes: earning deductions to finance benefits, and benefits that depend on earnings. This paper analyzes theoretically and empirically the trade-off between social insurance and incentive provision faced by reforms to these two attributes. First, I combine the social insurance and the optimal linear-income literature to build a model with a flexible pension contribution rate and benefits' progressivity that incorporates inter-temporal and inter-worker types of redistribution and incentive distortion. The model is general, allowing workers to be heterogeneous on productivity and retirement preparedness, and they exhibit present-focused bias. I then estimate the model by leveraging three quasi-experimental variations on the design of the Chilean pension system and administrative data merged with a panel survey. I find that taxable earnings respond to changes in the benefit-earnings link, future pension payments, and net-of-tax rate, which increases the costs of reforms. I also find that lifetime payroll earnings have a strong positive relationship with productivity and retirement preparedness, and that pension transfers are effective in increasing retirement consumption. Therefore, there is a large inter-worker redistribution value through the pension system. Overall, there are significant social gains from marginal reforms: a 1% increase in the contribution rate and in the benefit progressivity generates social gains of 0.08% and 0.29% of the GDP, respectively. The optimal design has a pension contribution rate of 17% and focuses 42% of pension public spending on workers below the median of lifetime earnings.

==> Income_pension_savings.tex <==
\begin{tabular}{lcccc} \hline
 & (1) & (2) & (3) & (4) \\
VARIABLES & log(Income) & log(Income) & log(Income) & log(Income) \\ \hline
 &  &  &  &  \\
\Delta\% Pension Savings & -0.094*** & -0.086*** & -0.083*** & -0.058** \\
 & [0.004] & [0.019] & [0.030] & [0.024] \\
 &  &  &  &  \\
Observations & 498,013 & 498,013 & 258,066 & 633,462 \\
R-squared & 0.086 & 0.347 & 0.346 & 0.082 \\
Age Controls & Yes & Yes & Yes & Yes \\
Other Controls & No & Yes & Yes & Yes \\
Crisis Definition & Long & Long & Long & Short \\
Sample Definition & Wide & Wide & Narrow & Wide \\
 Clustered SE & None & DoB-Sex & DoB-Sex & DoB-Sex \\ \hline
\end{tabular}


==> RDD_IV_rate_copy.tex <==
\begin{tabular}{lcccc} \hline
 & (1) & (2) & (3) & (4) \\
VARIABLES & log(Income) & log(Income) & log(Income) & log(Income) \\ \hline
 &  &  &  &  \\
Elasticity & -0.150*** & -0.144*** & -0.151*** & -0.149*** \\
 & [0.05] & [0.04] & [0.04] & [0.04] \\
 &  &  &  &  \\
Observations & 16,851 & 16,851 & 12,570 & 13,303 \\
Controls & No & Yes & Yes & Yes \\
Bandwith & Default & Default & Narrow & Donut-hole \\
 Clustered SE & DoB & DoB & DoB & DoB \\ \hline
\end{tabular}


==> RDD_IV_rate_copy_2.tex <==
\begin{tabular}{lccc} \hline
 & (1) & (2) & (3) \\
VARIABLES & log(earnings) & log(earnings) & log(earnings)  \\ \hline
 &  &  &    \\
 Post $\cdot$ Recipient$(=1)$& -0.0181*** & -0.0145*** & -0.0138***  \\
 & [0.002] & [0.002]  & [0.002]   \\
 &  &  &    \\
Observations & 281,106 &  281,106  & 140,553\\
R-squared & 0.053 & 0.182 & 0.192 \\
Controls & No & Yes & Yes \\
Bandwidth & 10\% & 10\% & 5\% \\
Clustered SE & DoB & DoB & DoB \\ \hline
\end{tabular}


==> first_stage.tex <==
\begin{tabular}{lccc} \hline
 & (1) & (2) & (3) \\
VARIABLES & Future Pension & Future Pension & Future Pension \\ \hline
 &  &  &  \\
money\_return\_FC3 & 0.814*** & 0.807*** & 0.856*** \\
 & [0.008] & [0.008] & [0.011] \\
 &  &  &  \\
Observations & 70,759 & 70,759 & 48,026 \\
R-squared & 0.560 & 0.566 & 0.557 \\
Age Controls & No & Yes & Yes \\
Other Controls & No & Yes & Yes \\
Crisis Definition & Short & Short & Long \\
Sample Definition & Narrow & Narrow & Narrow \\
 SE & Robust & Robust & Robust \\ \hline
\end{tabular}


==> health_pension.tex <==
\begin{tabular}{lccccc} \hline
 & (1) & (2) & (3) & (4) & (5) \\
VARIABLES & Health & Health & Health & Health & Health \\ \hline
 &  &  &  &  &  \\
Pension benefit & 0.311*** & 0.286*** & 0.286*** & 0.286*** & 0.343*** \\
 & [0.044] & [0.045] & [0.053] & [0.055] & [0.066] \\
 &  &  &  &  &  \\
Observations & 1,152 & 1,152 & 1,152 & 1,152 & 843 \\
Controls & None & Age-Gender & Age-Gender & Age-Gender & Age-Gender \\
SE & None & None & Robust & Cluster DoB & Cluster DoB \\
Crisis definition & Long & Long & Long & Long & Long \\
 Time retired & 0+ years & 0+ years & 0+ years & 0+ years & 3+ years \\ \hline
\end{tabular}

